Active Learning for Autonomous Intelligent Agents: Exploration, Curiosity, and Interaction

In this survey we present different approaches that allow an intelligent agent to explore autonomous its environment to gather information and learn multiple tasks. Different communities proposed different solutions, that are in many cases, similar and/or complementary. These solutions include active learning, exploration/exploitation, online-learning and social learning. The common aspect of all these approaches is that it is the agent to selects and decides what information to gather next. Applications for these approaches already include tutoring systems, autonomous grasping learning, navigation and mapping and human-robot interaction. We discuss how these approaches are related, explaining their similarities and their differences in terms of problem assumptions and metrics of success. We consider that such an integrated discussion will improve inter-disciplinary research and applications.

==> background.tex <==
	
%\section{Learning and Developing Agents}
%\label{sec:LearningAndDevelopingAgents}

%In this section we will present an overview of the many challenges faced by learning robot and agents. The reader will gain a general perspective of the supporting concepts and also understand why the problems faced by active agents cannot be solely seen in the same perspective as typical machine learning problems. Although machine learning techniques and results are at the core of the problems, there are many distinctive features when applying those methods to learning agents. We will start by discussing the learning problems that have been, and are being, addressed in robotics and also the main active learning principles from machine learning. Then we will generalize the active learning problem and show how the exploration problem is, in most cases, more specific to the robotics domain. This part will provide a general overview of all existing active approaches. Finally we will discuss the differences between active learning and curiosity and intrinsic motivation systems, and present the interactive learning problem and the active perception.




%\subsection{Exploration and Learning}
%\label{sec:ActiveLearningSettings}
%
%In this review we take a very broad perspective on the meaning of active learning. We consider any case where the agents \textit{actively} looks for the data instead of waiting to receive it. Under this perspective we can include different approaches that are given different names in different communities. Readers familiar with the exploration/exploitation problem might already have noticed that in robots the problem is more complicated than the typical AL setting in the machine learning community.
%
%We will give a running example of the general problem that it is intuitive and simple enough but includes all aspects of the general problem. We can think of a team of robots that wants to map a region and measure some physical quantities in the whole space. 
%
%At each time instant the robots must decide where to go next and what sensing action to use. To make this decision it is necessary to take into account the following aspects:
%
%\begin{itemize}
%	\item information value
%	\item cost of acquiring the information
%	\item cost of planning
%	\item cost of moving to the respective location
%	\item information gain over the planned path
%\end{itemize}
%
%A machine learning perspective on active learning does not consider the \textit{moving} problem and can just consider the value of information and eventually the cost of obtaining such information \cite{settles2008active}\footnote{In machine learning there also different settings of active learning namely \cite{}: pool based, sequential, synthetic samples, among others}. In robots, or agents, the physical limitations create these new constraints that will require particular attention. To note that this is not just a practicality as the problem of planning taking into account the costs and information becomes computationally harder, see for instance \cite{}. Figure \ref{fig:pathplan} summarizes this difference and latter on we will refer to this distinction to clarify the differences among the different methods.
%
%On the other hand exploration-exploitation strategies that consider the \textit{moving problem} do not consider the cost of information acquisition and assume a constant and uniform information value, see for instance R-Max \cite{}. More integrated perspective are starting to be addressed \cite{}.
%an early thesis on learning considering the cost of acquiring the data, planning to get there, quality of learning \cite{tan1991cost}
%SLAM path planning taking into account gains and observability \cite{Bryson08AES}
%
%\begin{figure}[htbp]
%	\centering
%		\includegraphics[width=0.7\columnwidth]{figures/pathplan}
%	\caption{Three perspective on active learning. A robot might choose: a) to look for the most informative path, ignoring the travel and data acquisition cost and the information gathered on the way there, b) to take into account the cost of acquiring the best point and c) consider the best path including the cost and the information on the way.}
%	\label{fig:pathplan}
%\end{figure}
%
%Until now we talked about the information value of single points. The name ''points'' comes from an analogy with the active learning in classification where points from a feature space are selected from. Nevertheless, in robots we can think about other perspective for selecting
%the \textit{most informative point}. Continuing with the same example, a robot might try to select particular locations that can provide more information but it might need to select between different regions, e.g. starting to map the beach or the forest. More abstract ideas can also be considered. The robot might decide that it is even more efficient to request a helicopter survey of a particular location, or decide which sensor to use. Here the robot is considering a selection among different exploration. A similar perspective is when the robot has to select among different learning methods or representations that can be more informative \cite{}. 
%The following list includes the possible choices that the learner might have available:
%
%\begin{itemize}
%	\item Selects points/trajectories
%	\item Selects among finite regions
%	\item Select exploration method
%	\item Select learning methods/representations
%\end{itemize}
%
%Note that the different communities have considered these possibilities in separate. AL learning typically considers choosing between points \cite{}, intrinsic motivation and optimal sensing has considered choosing among a finite set of regions \cite{}, and recently it has been considered how to choose online the best active learning method \cite{} or any other type of portfolio optimization \cite{}, in the people have consider the exploration-exploitation method without knowing the correct representation \cite{} and an integrated perspective of the three last problems has been introduced under the name of the strategic student problem \cite{}.
%
%A difficult problem is on how to compare and evaluate active learning. Typically it is a compromise between the data required and the quality of the learning. Measures can include: the average regret \cite{} where there is no distinct learning and testing phases and the regret is evaluated as the difference between the obtained reward and the maximum possible one. A simple regret measure \cite{} considers just the error in reward after learning. While a pure learning perspective would evaluate the average fit of the learning task \cite{}. If we consider fixed budget problems then more dimensions of evaluations would be required.
%
%
%
%
%For the pure learning problem of multi-armed bandits, where everything can be learned, regret bounds can be made \cite{Carpentier11ActMAB,gabillon2011MABident}.
%
%
%




==> deleted.tex <==
In terms of computational complexity, the shape of the reward does not change the convergence rate of the system but in practice there are several ways to improve the speed of learning: reward shaping \cite{Ng99rewshap}, optimistic initializations \cite{}, ... 




The concept of \textit{active imitation} discussed by \cite{Bandera07robotlearning}, follows previous works of \cite{demiris02imitationdualroute,macl05smc}, and consider the case where imitation is not just a passive recognition but instead a process where the motor system is involved in the recognition process, similar to the idea of motor theories of perception \cite{}.



passive map learning, links to some active  ???? \cite{koenig1996unsupervised}


==> imitation.tex <==
In any case, it is often not clear whether imitation concerns the motor intention or the underlying goal of that motor intention \cite{macl09ab,billard04discovering,RByrne99stringparsing,schaal99is}. In other words, it is often the case that the agent cannot unambiguously identify whether it should imitate the action, its outcome, or the reason driving the demonstrator to do it. In each of the following sections we we discuss in detail each of these three approaches to imitation learning. In particular, we refer to Section~\ref{Sec:infer} for a more detailed discussion on the problem of inferring the goal behind a demonstration. In that section we survey several recent works in which a learner does infer the goal of the demonstrator and adopts this goal as its own \cite{alissandrakis02alice,jansen06inferringintetion,macl07affimit,tenenbaum06actionunderstanding,rao07bayesianmodelimitation}.

%\subsection{Imitation in Natural Systems}
%\label{Sec:Biologicalevidence}
%
%The idea of learning by imitation has a clear inspiration in the way humans and other animals learn. Therefore, results from neurophysiology and psychology on imitation in humans, chimpanzees and other primates are a valuable source of information to better understand, develop and implement artificial systems able to learn and imitate. Section~\ref{Sec:Neurophysiology} details information from neurophysiology and Section~\ref{Sec:Psychology} presents evidence from psychology and biology. Such results illustrate the highly complex task that imitation is. The brief literature review in this section identifies some of the the problems that must be addressed before robots can learn (efficiently) by imitation and some works in the robotic literature that seek to model/test cognitive hypothesis.
%
%Neurophysiology identified several processes involved in action understanding that, in turn, contributed differently to the development of learning approaches in robotics. For example, mirror neurons \cite{gallese96actrecognition,Oztop06mirrorreview} provided an significant motivation for using motor simulation theories in robotics. Similar ideas were suggested in speech recognition \cite{Liberman85motortheory,Galantucci06motortheory}. Also the existence of forward and backward models in the cerebellum gave further evidence that the production system is involved in the perception, although it is not clear if it is necessary \cite{Wolpert98forbackmodels}. Most of these methods consider already known actions and not the way such knowledge can be acquired (we refer to \cite{Oztop06mirrorreview} for further discussion). For the case of novel actions there is evidence that the mirror system is not sufficient to explain action understanding and a reasoning mechanism must be involved \cite{brass07inferentialvssimulation}. We now discuss several of these views in more detail.
%
%\subsubsection*{Motor Theories of Perception}
%\label{sec:MotorTheoriesOfPerception}
%
%Several theories already claimed that the motor system is involved in perception. An example is the motor theory of speech perception \cite{Liberman85motortheory}. The three main claims in this theory are: ``(a) speech processing is special,
%(b) perceiving speech is perceiving gestures, and (c) the motor system is recruited for perceiving speech''. In \cite{Galantucci06motortheory}, the authors revisit such theory taking into account the results from the last $50$ years. The authors argue that although claim~(a) is likely false, claims~(b) and (c) are still likely to be true, although they admit that most of the findings supporting such claims may be explained by alternative accounts.
%
%One evidence in favor of the theory that the motor system is involved in perception is the existence of several mechanisms in the brain involved in motor prediction and reconstruction. One such mechanism depends on the existence of several pairs of forward and backward models in the brain \cite{Wolpert98forbackmodels}. The forward model codes the perceptual effects of motor actions, while the backward model represents the inverse relation, i.e. the motor actions that might cause a given percept. These models provide the agent with ``simulation capabilities'' for its own body dynamics, and are thus able to adapt to perturbations. They are also general enough to take into account task restrictions.
%
%\subsubsection*{Mirror and Canonical Neurons}
%
%The discovery of \emph{mirror neurons} \cite{gallese96actrecognition,fadiga97objectrepresentation,Oztop06mirrorreview} fostered a significant interest on the brain mechanisms involved in action understanding. These neurons are located in the F5 area of the macaque's brain and discharge during the execution of hand/mouth movements. In spite of their localization in a pre-motor area of the brain, mirror neurons fire both when the animal performs a specific goal-oriented grasping action and when it sees that same action being performed by another individual.
%%
%This observation suggests that the motor system responsible for triggering an action is also involved in the recognition of the action. In other words, recognition may also involve motor information, rather than purely visual information. Furthermore, by establishing a direct connection between gestures performed by a subject and similar gestures performed by others, mirror neurons may be related to the ability to imitate found in some species \cite{rama}, establishing an implicit level of communication between individuals.
%
%\emph{Canonical neurons} \cite{fadiga97objectrepresentation} have the intriguing characteristic of responding when objects that afford a \emph{specific} type of grasp are present in the scene, even if the grasp action is not performed or observed. Thus, canonical neurons may encode object affordances, as introduced in \cite{gibson79ecological}, and may help distinguishing ambiguous gestures during the process of recognition. In fact, many objects are grasped in very precise ways that allow the object to be used for specific purposes. A pen is usually grasped in a way that affords writing and a glass is held in such a way that we can use it to drink. Hence, by recognizing an object that is being manipulated, it is also possible to attain information about the most likely grasping possibilities (expectations) and hand motor programs, simplifying the task of gesture recognition.
%
%\subsubsection*{Reasoning Processes}
%\label{sec:ReasoningProcesses}
%
%Even if there is strong evidence that the motor system is involved in perception, it is not clear how fundamental it is and many claims on the mirror system are unlikely to hold \cite{Gopnik07mirrormyth}. For instance, mirror neurons are not strictly necessary for action production as their temporal deactivation does not impair grasping control but only slows it down \cite{fogassi01reachgrasp,Oztop06mirrorreview}. On the other hand, more complex mechanisms than mirroring are necessary to understand unexpected behaviors of an agent. In \cite{brass07inferentialvssimulation} an experiment is presented where a person turns a light on using its knee. Similar demonstrations are shown where the person has the arms occupied with a folder, many folders or none. Results from an \textit{fMRI} scan showed that the mirror mechanism is active during the empty arms situation (expected behavior) but it is not active during the other situation (unexpected behaviour). This and other similar results suggest that action understanding in unexpected situations is achieved by an inference-based mechanism taking the contextual constraints into account. In turn, this indicates that there may exist a reasoning mechanism to understand/interpret the observed behaviors.
%
%\subsection{Psychology}
%\label{Sec:Psychology}
%
%Studies in behavioral psychology have evidenced the ability of both children and chimpanzees to use different ``imitative'' behaviors. Individuals of both species also seem to switch between different such behaviors depending on perceived cues about the world \cite{horner05box,gergely02imitation}. These cues include, for example, the inferred purpose of the observed actions \cite{bellagamba99intention,johnson01infergoals,bekkering00imitgoal} even when the action fails \cite{want01mistakes,meltzoff95intentions,johnson01infergoals}. Other social learning mechanisms are analyzed in \cite{zentall01imitationmech} under the more general designation of \emph{social influence/learning}. In the continuation, we discuss some examples of behavior switching identified in the literature.
%
%\subsubsection*{Imitation Capabilities and Behaviour Switching}
%\label{sec:ImitationCapabilitiesAndBehaviourSwitching}
%
%\emph{Imitation} and \emph{emulation} are two classes of social learning mechanisms observed in both children and apes \cite{whiten04apesape,want02childrenape,tennie06}.%
%\footnote{Other species, such as dogs, have also been shown to switch strategies after having observed a demonstration, as seen in \cite{range07imitationdogs}.} In imitation, the learning individual adheres to the inferred goal of the demonstrator, eventually adopting the same action choice. In emulation, on the other hand, the individual focuses on the observed \emph{effects} of the actions of the demonstrator, possibly reaching these using a different action choice. The predisposition of an individual to imitate or emulate can thus be confirmed in tasks where the same effect can be achieved using different actions/motor patterns. For example, both chimpanzees and children are able to copy the choice of a push or twist movement in opening a box \cite{gomez96fruitprocessing}. 
%
%Children, in particular, can be selective about which parts of a demonstration to imitate \cite{gergely02imitation,williamson06goals}, but are generally more prone to imitate than to emulate. For example, children can replicate parts of a demonstration that are clearly not necessary to achieve the most obvious goal -- a phenomenon known as \emph{over-imitation} \cite{horner05box}. Over-imitation can be diminished by reducing the social cues or by increasing the urgency of task completion \cite{mcguigan07box35yrs,brugger07imitation,lyons05overimitation}. It has also been argued that over-imitation can occur for a variety of social reasons \cite{nielsen06} or because the individuals interpret the actions in the demonstration as causally meaningful \cite{lyons05overimitation}. 
%
%\subsubsection*{Sensitivity to Task Constraints}
%\label{sec:SensitivityToTaskConstraints}
%
%Social animals also exhibit some sensitivity to the context surrounding the task execution, particularly task constraints. For example, in \cite{meltzoff88imitatiom} 14-month-olds were shown a box with a panel that lit up when the demonstrator touched it with his forehead.%, to test infants' memories of novel actions. 
%The results showed that most infants reproduced the use of the forehead rather than using their hand when presented with the object a week later. This experiment was further extended in \cite{gergely02imitation} by including a condition in which the demonstrator was restricted and could not use her hands. It was observed that only $21\%$ of the infants copied the use of the forehead, against the $69\%$ observed in a control condition replicating the \cite{meltzoff88imitatiom} study. It was argued that, in the latter condition, infants recognize no constraints upon the demonstrator and thus encode the use of the forehead as a specific part of the intention. In the restricted case, they recognize the constraint as a extraneous reason for the use of the forehead and do not encode the specific action as part of the intention.
%
%We return to this particular experiment in Section~\ref{Sec:infer}, in the context of computational models for social learning.
%
%\subsubsection*{Imperfect Knowledge}
%\label{sec:ImperfectKnowledge}
%
%Several experiments were conducted to investigate how the knowledge about the world dynamics influences social learning mechanisms. In one archetypical experiment, an individual observes a sequence of actions, not all of which are actually necessary to achieve the outcome. For example, in \cite{horner05box}, preschoolers and chimpanzees were presented with two identical boxes, one opaque and one transparent. A demonstrator then inserted a stick into a hole on the top of the box and then into another hole on the front of the box. It was then able to retrieve of a reward from the box. In this experiment, the insertion of the stick into the top hole was unnecessary in order to obtain the reward, but this was only perceivable in the transparent box. The results showed that 3 and 4-year-old children tended to always imitate both actions. On the contrary, chimpanzees were able to switch between emulation and imitation if causal information was available: after having observed demonstrations in a transparent box, the chimpanzees were much less prone to insert the stick into the upper (useless) hole.
%
%\subsubsection*{Goal Inference}
%\label{sec:GoalInference}
%
%Finally, it has been showed that some species exhibit imitative behavior beyond simple motion mimicry. For example, primates tend to interpret and actually reproduce observed actions in a teleological manner -- that is, in terms of the inferred goals of the action \cite{csibra07teleological}. In an experiment designed to test this hypothesis, 3 to 6-year-old children observed a demonstrator reaching across her body to touch a dot painted on a table to one side of her, using the hand on her other side \cite{bekkering00imitgoal}. When prompted to reproduce the observed demonstration, children tended to copy the dot-touching action, but not the use of the contra-lateral hand. However, when the same demonstration was performed without a dot, children tended to imitate the use of the contra-lateral hand. It was argued that, in the first case, children interpreted the dot touching as the intention, choosing their own (easier) way to achieve it, while in the second case there was no clear target of the action but the action itself. As such, children interpreted the use of the contra-lateral hand as the intention and imitated it more faithfully. Results in experiments adapted for older children infants are similar \cite{carpenter05goals}.
%
%\subsection{Visual Transformations}
%
%The same motor action can have very distinctive perceptual results if one considers different points-of-view. For example when a person gestures goodbye, she can see the back of her hand, while when someone else is doing the same she will see the palm of the other's hand. This poses a problem when mapping actions from the demonstrator to the learner, as already identified in \cite{bruner72vpt} and depicted in Fig.~\ref{fig:alloegofmelo}.
%
%\begin{figure}[!tb]
%	\centering
%		\includegraphics[width=0.7\textwidth]{alloegofmelo}
%	\caption{Perceptual difference between the same gesture having an ego- or an allo- perspective.}
%	\label{fig:alloegofmelo}
%\end{figure}
%
%The typical solutions for this problem is to perform a complete three-dimensional reconstruction. However, several works proposed alternative approaches that consider simplifications to such problem. In \cite{Bandera07robotlearning,gardner02perspective,asada00without3d,macl03vistransgest,macl05smc} several transformations are discussed, ranging from a simple image transformation (\eg mirroring the image) to a partial reconstruction assuming an affine camera and the full three dimensional reconstruction. These works also point out that such transformations can be seen as imitation metrics, because the depth information in some gestures can indeed change the meaning of the action. Such transformations can also be done using neural networks \cite{billard05framecorrespondence}.
%
%\subsection{Mimicking Behaviors and Automatic Imitation}
%
%Several works on imitation seek to transfer behaviors by a simple motor resonance process. The observation of perceptual consequences of simple motor actions can elicit an automatic mimicking behavior, and several initial works on imitation adopted this approach \cite{demiris94imitcontroller,demiris96imitative,demiris97head,gaussieretall97percepacitonloops}. In these works, the relation between changes in perceptual channels caused by a demonstrator are directly mapped into motor actions of the learner. Particularly in \cite{demiris96imitative}, the orientation of a mobile robot is controlled according to the observed position and orientation of a human head.
%
%In these approaches the model about the own body is not explicit, the relations between action and perception is learned without concern about the true geometry and dynamics of the body.
%
%Using the visual transformations introduced earlier it is possible to generate more complex behaviors. In \cite{macl03vistransgest,macl05smc}, the learner starts by acquiring a correspondence between its own perceptions and actions. The mimicking behavior results from mapping the perception of the demonstrator to its own using a view-point transformation, and then activating an inverse sensory-motor map. Different visual transformations result in different types of behavior.
%
%Examples of other methods posing imitation within this visuo-somatic perspective include \cite{Asada06visuosomaticmap,gaussieretall97percepacitonloops}. An interesting approach is proposed in \cite{Boucenna08face} where facial expression are learned by interacting with a person and creating a resonance of expressions.
%
%\subsection{Imitation through Motor Primitives}
%
%All previous approaches consider a simple perception-action loop in imitation. However, when considering a learner equipped with several motor primitives, it is possible to achieve more complex interactions. The ``recognition'' block in Fig.~\ref{fig:imitarch} represents the translation of observed trajectories in terms of such motor primitives. A motor sequence is perceived, maybe after some visual processing, and recognized as a specific motor primitive \cite{maistros01percactimitation,mataric02smm}. This general approach can be used to perform human-machine interaction \cite{breazeal99imitation} or to learn how to sequence such primitives \cite{RByrne99stringparsing}. 
%
%In \cite{RByrne99stringparsing} a string parsing mechanism is proposed to explain how apes are able to learn by imitation to process food. The string parsing mechanism is initialized with several sequences of primitives. Learning and generalization are performed by extracting regularities and sub-sequences. This approach can be seen as a grammatical inference process.
%
%Other approaches use hidden Markov models to extract such regularities and filter behavior, usually in the context of tele-operation. The main goal of such approaches is to eliminate sluggish motion of the user and correct errors. We refer to \cite{yangteal96hmmtelerobotics} for an application of one such approach to the control of an Orbit Replaceable Unit. In this work, a robot observes an operator performing a task and builds a hidden Markov model that describes that same task. In \cite{hovland96skillacq}, a similar approach is used in assembly tasks. Such models can also be used to detect regularities in human motion \cite{Calinon07chapter}.
%
%Regularities of human motion can be represented in low-dimensions using principal component analysis \cite{Chalodhorn09imitateeigen}, clustering \cite{Kulic09motorprimitives} or other non-linear manifold learning techniques \cite{Jenkinsetal2006icdl}.
%
%Some authors rely on completely separated methods to recognize and to generate motor primitives. Others combine both processes, thus exploring the self-modeling phase \cite{chadwickeetal00primitivebased,demiris06hammer,macl05smc,demiris02imitationdualroute}. As seen in Section~\ref{Sec:Neurophysiology}, this process can be explained by the use of motor simulations of some kind. For example in both \cite{demiris06hammer} and \cite{Wolpert03unifying}, action recognition is performed using the idea of coupled forward/backward models discussed in \cite{Wolpert98forbackmodels}. The former decouples each of the action primitives and is thus able to deal with a larger variety of tasks, while the latter is able to combine several primitives and deal with complex motor skills in a robust way. In \cite{Erlhagen06a,Erlhagen06b} dynamic neural networks are used to recognize actions goals taking into account task restrictions. A single neural network able to encode several behaviors was introduced in \cite{Tani04mirrorRNNPB} and performs similar computations.
%
%\subsection{Learning of New Task Solutions}
%
%In some cases the learner has an explicit goal. However, it might be very difficult to plan how to reach such goal. This is specially important in complex environments or in situations involving highly redundant robots (\eg humanoid robots). One of the main motivations behind imitation learning is that it provides an easy way to program robots. Therefore, most approaches to imitation consider the learning of new actions. In such approaches two main trends have been adopted: one considers many demonstrations of the same task and tries to find invariants in the observed motions \cite{billard04discovering,rao07bayesianmodelimitation}. The other uses only the observed trajectories as an initialization and then improves and generalizes further (\eg using reinforcement learning) \cite{Peters05ecml}.
%
%In \cite{price03rlimit}, imitation is used to speed up learning and several metrics were defined for evaluating the improvement in learning when using imitation. Imitation is used in \cite{Schaal03learnprimit} to learn dynamic motor primitives. As argued in this work, ``\textit{Movement primitives are parameterized policies that can achieve a complete movement behavior}''. From this perspective, motor primitives can be seen as dynamical systems that generate different complex motions by changing a set of parameters. The authors also suggest the use of data from a demonstration to initialize such parameters. The parameters can then be optimized using, for example, policy gradient \cite{Peters05ecml}. We point out that these methods consider classes of parameterized policies, namely the parameters of the dynamical system.
%
%One of the few approaches taking uncertainty into account is proposed in \cite{Grimes07NPImitation}. The approach in this work starts by learning a Gaussian mixture model as a forward model, using self-observation \cite{Shon05GPimitation}. The demonstration is taken as observation of a probabilistic process and the goal is to find a sequence of actions that maximizes the likelihood of such evidence. The work focuses on copying motions taking into account the dynamics of the robot and, as such, uses as observations the estimated state trajectory and ignores the dynamic information. It achieves body correspondence by inferring the most probable trajectory using the imitator's body. Extra task restrictions can also be included. In \cite{Chalodhorn09imitateeigen} walking patterns are transferred from humans to robots after adapting it for different kinematics using low level representations.
%
%Finally, several other methods are agnostic as to what is exactly the goal of the demonstrated task and aim only at learning the observed course of action. For example, in \cite{Chernova09jair}, learning from demonstration is formulated as a classification problem and solved using support-vector machines. These methods, in a sense, disregard the effects and social context of the demonstration, and focus only on replicating in each situation the demonstrated course of action (see Section~\ref{Sec:infer} for a more detailed discussion on this). One disadvantage of this general approach is that it places excessive confidence on the demonstrator. Furthermore, the course of action learned is specific to the context and environment of the learner and, as such, is not generalizable to different environments.
%

\subsection{Imitation in Artificial Systems}
\label{sec:imitproblems}

Imitation learning brings the promise of making the task of programming robots much easier \cite{schaal99is}. However, to be able to imitate, robots need to have several complex skills that must be previously implemented or developed \cite{macl07smc}. 


In \cite{Wolpert03unifying}, the authors identified three subproblems (or classes thereof) to be addressed in developing one such system:
%
\begin{itemize}
\item Mapping the perceptual variables (\eg visual and auditory input) into corresponding motor variables;
\item Compensating for the difference in the physical properties and control capabilities of the demonstrator and the imitator; and
\item Understanding the intention/purpose/reason behind an action (\eg the cost function to be minimized in optimal control that determines the action to be taken in each situation) from the observation of the resulting movements.
\end{itemize}
%
If we further take into account that the perceptual variables from the demonstrator must also be mapped from an allo- to an ego- frame of reference, the first of the above subproblems further subdivides into two other sub-problems: view-point transformation and sensory-motor matching \cite{bruner72vpt,asada00without3d,macl03vistransgest,macl05smc,billard05framecorrespondence}. The second of the problems referred above is usually known as the \emph{body correspondence problem} \cite{nehaniv98mapping,alissandrakis06correspondence,nakaoka03stabledance} and is, in a sense, closely related and dependent on the first problem of mapping between perception and action. 

\subsubsection*{Data Acquisition}
\label{sec:DataAcquisition}

The way to address the issues discussed above will largely depend on the context in which imitation takes place. When used for robot programming, it is possible to use {\em data acquisition} systems that simplify the interpretation and processing of the input data, thus reducing partial observability issues. The latter is important since the learner will seldom be able to unambiguously observe all the relevant aspects of the demonstration. In particular, this can allow more robust and efficient algorithms to tackle the allo-ego transformation, the perception-to-action mapping and the body correspondence. 
%
Examples of such systems include exoskeletons, optical trackers or kinesthetic demonstrations \cite{Billard07PbD}.

Other applications of imitation occur in less controlled environments, for example as a result of the natural interaction between a robot and a human. In such contexts, perceptual problems must be explicitly addressed. Some authors address this problem adopting a computer vision perspective \cite{macl03vistransgest}, modeling partial observability \cite{Doshi08actpomdp} or being robust to noise in the demonstration \cite{Ramachandran07ijcai,macl07affimit,macl09poirl}.

\subsubsection*{Mapping of Perceptual Variables and Body Correspondence}
\label{sec:MappingOfPerceptualVariables}

Many approaches do not consider a clear separation between data acquisition and learning by demonstration. One way to deal with the lack of information/data is to use prior knowledge to interpret the demonstration. {\em Action interpretation} strongly depends on the knowledge about how the world evolves as well as on the capabilities of both the learner and the demonstrator to interact with it \cite{gergely02imitation,horner05box,macl09ab}. %
This process is closely related with the two first issues pointed out in \cite{Wolpert03unifying}, since it provides a way to map external inputs to internal motor representations (\eg to robot actions). Therefore, imitation learning algorithms will typically benefit from prior knowledge about the environment, specially when data acquisition cannot provide a full description of the demonstration. 

Knowledge about the agent's own body and its interaction with the world simplifies some of the difficulties found in imitation. On one hand, for the perception-to-action mapping, the recognition of others' actions can rely on the learner's model of the world dynamics, \eg by inferring the most probable state-action sequence given this model. This idea draws inspiration from psychological and neurophysiological theories of motor perception, where recognition and interpretation of behavior are performed using an internal simulation mechanism \cite{arbibetall00brainimag,gallese96actrecognition,macl05smc}. As seen in Section~\ref{Sec:Biologicalevidence}, mirror neurons are one of such mechanisms \cite{gallese96actrecognition}, and a significant amount of research in imitation learning in robotics flourished from this particular discovery.

On the other hand, this type of knowledge also allows action recognition and matching to occur with an implicit body correspondence, even if the bodies of the learner and demonstrator are different. Several works have explored this idea. For example, in \cite{nehaniv98mapping,nakaoka03stabledance,Shon05GPimitation,Shon07imitmultdemons,macl03vistransgest,macl05smc}, action matching is addressed at a trajectory level. In these works, the demonstration is interpreted taking into account the different dynamics of the learner and the demonstrator. In \cite{macl08affTRO,montesano07icdl,kozima02imitation}, the same problem is addressed at a higher level of abstraction that considers the \emph{effects} on objects. 

\subsubsection*{Goal/Intention Inference}
\label{sec:GoalIntentionInference}


Identifying the goal driving a demonstration is a particularly complex inference process, indeed an 
ill-defined one. What to imitate depends on several physical, social and psychological factors (see Section~\ref{Sec:Psychology}). One possible way to answer this question relies on the concept of \emph{imitation metrics}. These metrics evaluate ``how good'' imitation is. Imitation metrics were first explicitly introduced in \cite{nehaniv01measures} in order to quantify the quality of imitation, to guide learning and also to evaluate learned behavior. However, it is far from clear what ``good imitation'' is and, perhaps more important, how variable/well-defined the learned behavior can be. Some studies along this direction have characterized the quality of imitation in humans. In \cite{pomplun00metric}, subjects were asked to perform imitation tasks and quantitative results were obtained to assess the effect of rehearsal during observation and repetition of the task.


\subsubsection*{The Role of Self-Observation}
\label{sec:TheRoleOfSelfObservation}

It is interesting to note that most of the necessary information about the robot's body and the world dynamics can be gathered by self-observation \cite{macl07smc,yiannis05babbling}. Although slow in many situations, it often allows a greater adaptation to changing scenarios.

Many different techniques can be used by the robot to learn about its own body \cite{Schaal03learnprimit,aaronetall01learninvkin,macl07smc,peters08motorskills,Wang08GPMotion}. For example, several works adopt an initial phase of motor babbling \cite{kuniyoshi03smmimitation,macl05smc,macl07smc,Grimes07NPImitation}. By performing random motions, a great amount of data becomes available, allowing the robot to infer useful relations about causes and consequences of actions. These relations can then be used to learn a body schema useful in different application scenarios. The specific methods used to learn body models vary, and range from parametric methods \cite{micha08bodyschema,macl09bodyschema}, neural network methods \cite{kuniyoshi03smmimitation,macl03vistransgest,macl05smc} to non-parametric regression \cite{aaronetall01learninvkin,Wang08GPMotion,macl07smc} and graphical models \cite{burgard08bodyschema,Grimes07NPImitation}. As for learning about the world dynamics, this is closely related to the concept of learning affordances. Repeated interaction with the world allows the robot to understand how the environment behaves under its actions \cite{macl08affTRO,macl07aff,metta03poking,Sahin07}. 
As seen in the previous section, the knowledge about the world dynamics and the capabilities of others strongly influences how actions are understood.

$$\diamondsuit$$



For example, in \cite{Ratliff06icml}, learning from demonstrated behavior somewhat resembles transfer learning, in which an agent observes demonstrations in different scenarios and uses this knowledge to recover a reward function that can be used in yet other scenarios. This problem is addressed as a max-margin structured learning problem to recover a reward function from a set of demonstrations. In order to simplify the problem and to leverage fast solution methods, the paper formulates the problem as a non-linear (non-differentiable) unconstrained optimization problem, that is tackled using subgradient techniques that rely on the solution structure of the (embedded) constraints.

In \cite{nadel01repeated,nadel02imitation}, robots able to imitate have been used to interact with autistic children. On a related application, the Infanoid project \cite{kozima00infanoid,kozima03keepon} deals with gesture imitation
\cite{kozima02imitation}, interaction with people \cite{kozima01autism}, and
joint attention \cite{nagai02develjoint}. The robots in this project are used in human-robot interaction scenarios with particular emphasis on people with special needs. Although the results seem promising, and in short term people seem to react well, care must be taken in ensuring that the robots are used to promote socialization with other people, and not a stronger focus on the machine itself \cite{Robins05robotsautismcautionary}.

Some authors have also addressed imitation in multiagent scenarios, considering multiple demonstrators \cite{Shon07imitmultdemons}, multiple learners \cite{Chernova08multiplelfd} and human-robot joint work \cite{Erlhagen07jointtask}. In the presence of multiple demonstrators, these may be performing different tasks and the agent must actively select which one to follow. In \cite{Shon07imitmultdemons}, this observation led the authors to call their approach \emph{active imitation}.


Understanding actions and inferring intentions generally requires a more explicit reasoning process than just a mirror-like mechanism \cite{brass07inferentialvssimulation}. As discussed in Section~\ref{Sec:Biologicalevidence}, by further abstracting the process of learning by imitation to \emph{task level} it is possible to additionally include contextual cues \cite{macl09ab,tenenbaum06actionunderstanding,jansen06inferringintetion}. At this level of abstraction the third issue identified in \cite{Wolpert03unifying} becomes particularly relevant. 


Computational models of imitation have also been proposed to understand biology by synthesis. Examples include models of language and culture \cite{alissandrakis04robotcultures,Billard99protolanguage}, curiosity drives resulting in imitation behaviors \cite{Kaplan07imitationmotiv}, behavior switching in children and chimpanzees \cite{macl09ab}. 

We also note that there are other social learning mechanisms that fall outside the ``imitation realm'' in biological research. Often imitation is seen as a fundamental mental process for acquiring complex social skills but other mechanisms, although cognitively simpler, may have their own evolutionary advantages \cite{Noble02sociallearning,fmelo07unified,Oudeyer03languagesimple}. 


==> index.tex <==
Proposed organization:

1- Intro:
a) Learning in robotics
b) need for active learning (AL)
c) AL in machine learning: basic stuff
d) Broadening AL: exploration/explotation, intrinsic motivation, social robots 


2 - Background
a) Theory for Active learning and its implications/limitations on robotic problems
b) Historical perspective on active learning on robotics (what problems: mapping, RL, manipulation, )

3- A taxonomy of active learning in robots
a) Example
b) Information and costs in robotic problems
c) What can be selected
d) A global perspective of active learning in robotics: AL, Explo/Explo, Intrinsic Motivation, Interactive Learning
e) Evaluation

From here on describe every item provided in the global perspective


Taxonomy:

Pre-defined tasks

A) learning through experience:
A.1) Active perception for building models (Regression and classification)
A.2) Exploration/Explotation (model free or model based):
- RL
- Policy gradient
A.3) Strategic student problem

Oracle based:
- Active (regression and classification)
- Interactive Learning 


Unknown tasks
- Curiosity.


Things I don't know where to put:
- Theoretical considerations
- Comparisions between approaches
- Old works


==> robotlearning.tex <==
\subsection{Learning robots: background and history}
\label{sec:learningrobots}

\todo{para reduzir o numero de referencias tentar trocar todos os exemplos por exemplos activos, eventualmente deixar os mais importantes nao activos}

early ideas of learning in robots comparison between strategies \cite{dorigo1994robot} to check better


Learning applied to robots already has a long story. An early book on robot learning \cite{connell1993robot} shows that most applications of learning to robots problems have been discussed long time ago. In the last two decades, however, there have been important changes from theoretical developments to increased computational power, that have altered the landscape of applications and possible solutions. A more recent survey can be found in \cite{schaal2002robot} where ***...***. There exist also other surveys focusing on specific problems (e.g. learning in control problems \cite{nguyen2011surveymodel}) or in subareas where learning robots play a central role (e.g. developmental robotics \cite{} and social robotics \cite{goodrich2007human}). Indeed, learning has been applied to almost every robotic problem previously addressed with non-learning approaches. Although the level of success of learning varies depending on the problem at hand, learning is becoming more and more conspicuous due to the increase on computational power, the limits of classical methods and the difficulty of designing good models for real open-ended dynamic environments.

It is out of the scope of this survey to review all applications of learning in robotics. However, to put active learning into context, it is necessary to give a brief overview of the problems and methods. Table \ref{tab:learningexamples} has a non-exhaustive list of examples of learning robots. It also shows the variety of methods and techniques that have been used which include simple classifiers, kernel methods, probabilistic representations. At the highest abstraction level, learning aims to estimate some kind of generic function (e.g. the boundary of a classifier, a policy, the free parameters of a parametric model for a transition, ...). What the function represents depends on the specific scenario and includes low level controllers, models of the environment, transition models, full trajectories, abstract discrete policies or strategies for interacting with humans.   

*** LUIS ATE AQUI ***

Early works include: learning locomotion reflexes: A self-supervised neural system for mobile robots \cite{dubrawski1994learning}, automatic robot programming based on inductive learning \cite{dufay1984approach}, robot trajectory learning through practice \cite{atkeson1986robot}, control \cite{moore1993fast}, robot juggling \cite{schaal1994robot}, automatic programming of behavior-based robots using reinforcement learning \cite{mahadevan1992automatic,gullapalli1994acquiring}.

What is learned depends strongly on the application and on the domain but has considered the techniques more common on machine learning such as regression \cite{sigaud2011regrsurvey,Nguyen-Tuong2008,montesano12actbetas}, classification \cite{sigaud2011regrsurvey}, clustering \cite{}, mixture models \cite{khansari2010bm}, general graphical models \cite{macl08affTRO}, reinforcement learning \cite{}, but also techniques more common from control theory and signal processing such as dynamical systems learning and identification \cite{nguyen2011surveymodel,khansari2010bm,macl06tseq,ko2009gp}, manifold learning \cite{peters05manifoldrobonaut,macl07manifold}.
In many situations learning is not done from self-exploration but by learning from looking at an human expert \cite{bakker1996robot}.

All these techniques results in dynamical models that can be used to control, plan \cite{kocijan2003predictive,ko2007gpblimp} and even recognize others \cite{wang2008gaussian}, filtering \cite{ko2009gp,kocijan2003predictive,ko2007gpblimp}, learn directly and action policy \cite{nguyen2011surveymodel}, interaction protocols \cite{macl11simul}, among many others. 

As most robot control is made doing model-based methods, several approaches consider how to learn such models from data. The seminal work from \cite{Ljung77TAC,ljung1999system} on system identification is probably the earliest theoretical approach of such problem. Recently black-box methods have been gathering more interest to model the more complex systems and application. Recent surveys include how regression models have been used to learn the dynamics of robots \cite{sigaud2011regrsurvey} or when applied to model-based control \cite{nguyen2011surveymodel}.


\cite{solis2007reactive}


\begin{table}[!t]%
\centering
\begin{tabular}{|l|l|l|} \hline
%% ORACLE FREE
%\multicolumn{3}{|>{\columncolor[gray]{.8}}c|}{Interactive learning. Active oracle.} \\ \hline
\rowcolor[gray]{.8} & Reference & Learning method\\
\multirow{2}{*}{Control} & *** & ** \\
& *** &  \\ \hline
\multirow{2}{*}{Navigation} & *** &  \\
& *** &  *** \\ \hline
\multirow{2}{*}{Mapping and localization} & *** &  ** \\
& *** &  \\ \hline
\multirow{2}{*}{Manipulation and grasping} & *** &  \\
& *** &  \\ \hline
%% ORACLE 
\multirow{2}{*}{Development} & *** &  \\
& *** &  \\ \hline
\multirow{2}{*}{Human-robot interaction} & *** & *** \\
& *** & *** \\ \hline
\end{tabular}
	
\caption{Examples of learning robot applications.}
\label{tab:apps}
\end{table}


==> teaching.tex <==
\subsection{Algorithmic Teaching}
\label{sec:Teaching}

\textit{Algorithmic teaching} (AT) formally studies the optimal teaching problem, that is, finding the smallest sequence of examples that uniquely identifies a target concept to a learner. Work within AT, tries to identify the teachability of different concept classes and devise efficient algorithms that produce optimal teaching sequences~\cite{Balbach09algteach,Goldman95,cakmak12algteach}. AT can be seen as a complementary problem from the active learning but here it is the teacher that is choosing its examples in an intelligent way. Algorithmic teaching gives insights into what constitutes informative examples for a learning agent. These insights can in turn be used by human teachers while training a learning agent to perform sequential decision tasks, e.g. a personal robot or virtual assistant.

With a human-in-the-loop the learning process can be faster 
Several authors, from different communities, have considered how to choose training programs that will speed up learning. Several heuristics have been proposed such as {\em starting small} \cite{elman93learning}, curriculum learning \cite{Bengio09curriculum}, maturation \cite{baranes2013active,} and development \cite{}. For instance, {\em curriculum design} suggests that the teacher should select examples by starting with {\em easy} examples and gradually increasing the difficulty \cite{elman93learning,Bengio09curriculum,zang10,taylor09}. This is analogous to the {\em scaffolding} behavior common in human teachers \cite{Mascolo05nip}. \cite{khan11nips} demonstrated that this is the most prominent strategy in human teaching and provided a theoretical account for it.
{\em Pedagogical sampling} assumes a benevolent teacher and learner; consequently the teacher chooses most informative examples for the learner \cite{shafto08cogsci,warner11cogsci}. In many cases, AT can provide theoretical results for different types of classification tasks with different assumptions on the learner and on the interaction protocol \cite{Balbach09algteach,Goldman95,Mathias97interteach,Natarajan87teachbool}.

teaching \cite{collins1993design}\cite{katagami2000real}\cite{calinon2007active}\cite{katagami2003active}\cite{thomaz2006reinforcement}


Other work on teaching takes a more human-inspired approach.


????? teaching \cite{Mathias97interteach}\cite{katagami2003active}



==> toadd.tex <==
\section{Stuff to add}


\todo{
learn representations 
\cite{nicolescu2001experience}

A tutorial on bayesian optimization of expensive cost functions, with application to active user
modeling and hierarchical reinforcement learning \cite{brochu2010tutorial}

Impact of Human Communication in a Multi-teacher, Multirobot Learning by Demonstration System \cite{martinsimpact}
}



Optimal experimental design \cite{}  \cite{Angluin88queries,Cohn96,Seeger08ICML,Castro2008}

Other alternative settings include KWIK learning \cite{li-littman-walsh-strehl:11-mlj} and XXXXXX \cite{}

However, there are also situations in which the agent sequentially learns while moving or acting in the environment, but its actions are completely decoupled from the learning process (e.g. robot map learning. In this latter situation the robot is not passive, but it is not necessarily actively looking for information but rather passively receiving it from the motion. 

put optimal teaching somewhere:::
 In this context, active learning has links with optimal teaching \cite{} and social interaction between the robot and the agent providing the information. 
	
Batch active learning \cite{chen13batchactivelearn}
active multi-objective \cite{zuluaga13activemultiobject}

\cite{chattopadhyay13transferandactive}

Sequential Bayesian Search \cite{wen2013sequential}

Optimal regret bounds for selecting the state representation in reinforcement learning \cite{maillard2013optimal}


\cite{whitehead1991study}
Two general cooperative mechanisms are described: Learning-with-an-ExternalCritic
(or LEC) and Learning- By-Watching (or LBW). Specific algorithms for each
are studied empirically in a simple grid-world and shown to improve significantly agent
adaptability.
Analytical results for both, under various learning conditions, are also provided.
These results indicate that while an unbiased search can be expected to require time
exponential in the size of the state space, the LEC and LBW algorithms require at
most time linear in the size of the state space and under appropriate conditions are
independent of the state space size and require time proportional to the length of the
optimal solution path.


Raghavan, H. and Allan, J. (2007). An interactive algorithm for asking and incorporating feature feedback into support vector machines. \cite{raghavan2007interactive}

Acquiring joint attention skills, i.e. being able to understand if someone is looking at the same objects as we, is a very important skills for many social situations. In the work of \cite{doniec2006active} the robot actively points towards objects thus guiding the learning process much faster.



maya hri 2012, includes links to active learning in robots


reviews bayesian and optimal experimental design

optimization methods used by Ruben \cite{}

abstract algorithms to check better \cite{moore2000q2}, \cite{sugiyama2000incremental}

language \cite{zhang2001grounded}\cite{andry2001learning}

mutual adaptation \cite{tani2008codevelopmental}



probably not 

One early idea applied interactive learning where a user would operate the robot with a joystick to teach it a topological map of the environment \cite{}.

This learning through interaction will allow a better acceptance of machines and a more widespread use, see \cite{Fong2003} for a survey of socially interactive robots. survey hri \cite{goodrich2007human}

learning from demonstration by viapoints adaptation \cite{miyamoto1996kendama}

Interactive multimodal robot programming.\cite{iba2005interactive}









\subsection{Active Learning}
\label{sec:ActiveLearning}



to add: theory \cite{Balcan2008,golovin10adaptive,golovin10near,Krause07,Schohn00}

\cite{roy2001toward}
Toward optimal active learning through monte carlo estimation of error reduction

\todo{ NOT SURE WHERE TO PUT THIS NOW. PROBABLY REMOVE
From the opposite direction the Algorithmic Teaching (AT) literature can provide some insights on the difficulty of learning. The goal of this field is to allow a teacher to select the examples enabling a learner to acquire a concept in polynomial time. An early computational measure was the Teaching Dimension \cite{Goldman95}, or its variants \cite{Natarajan87teachbool,anthony95,balbach08,Balbach09algteach}. These results are the proof that the sequence of training examples have a critical impact on the learning rate. Note that in the active learning problem it is the learner that chooses its samples. In many cases, a teacher that chooses examples optimally will teach a concept significantly faster than an active learner choosing its own examples~\cite{Goldman95}. Most results on AT were done to classification tasks but recent contributions started to explored more complex tasks such as markov decision processes \cite{cakmak12algteach}.
}


check:
An interesting extension was done by \cite{muslea2002active}. Here the authors consider situations where the features might consist in several disjoint datasets that can predict the correct label. An application in robotics consider for instance texture and color for terrain classification \cite{dima2005active}.









\subsection{PYOudeyer}
\label{sec:PYOudeyer}

Karl Friston

neuro-constructivism, Gerb Westerman, Sylvain Sirois, Denis Mareschal


\subsection{random stuff}
\label{sec:randomStuff}

%In robotics the idea was also proposed as early as \cite{}. \todo{Recently the applications of active learning have started to cover a larger extent of topics: body schema acquisition \cite{Cantin10icra}, grasping \cite{montesano12actbetas}, learning from demonstration \cite{macl09airl,melo2010metric}. Work on active learning has considered {\em confidence based autonomy}~\cite{Chernova09jair}, active inverse reinforcement learning \cite{macl09airl,cohn2011comparing} or eliciting reward queries \cite{regan2011eliciting}. }

%Learning through experience is inherently an active approach to learning and, consequently, has a large literature specially in the field of reinforcement learning through the development of different exploration and exploitation strategies \cite{}. 

Many of these methods are very inefficient in the use of the samples. Several authors considered the use of importance sample to reuse data from one policy to the other \cite{Melo08ecml}.

Being local methods the usual approach is to initialize a controller either using a simplified estimated model of the system \cite{} or by using trajectories obtained from human execution \cite{}.

These methods are the ones more used in robotic application that include high speed and difficult to model non-linearities. Examples range already from ball-in-cup \cite{}, grasping \cite{}, tennis playing \cite{}, walking \cite{nakanishi2004learning}, among others.

\cite{neumann2011variational,neumann2009learning,neumann2008batch}
\cite{daniel2012hierarchical,kober2011policy,kroemer2011active,peters2010relative,kober2009learning}

Pac-bayesian analysis of the exploration-exploitation trade-off \cite{seldin2011pac}

maybe for the imitation part
\cite{boularias2012structured,wang2011learning,kroemer2011active,boularias2011relative,piater2011learning,kroemer2010combining,kroemer2009active}

Learning from demonstration and adaptation of biped locomotion 
\cite{Peters05ecml}\cite{peters06policygradient}\cite{Peters06rss}\cite{peters08motorskills}


An interesting problem of how to acquire a database for learning faces is presented by \cite{hewitt2006active}. There the authors show that by using face detection and tracking it is possible to continuously acquire a sufficiently varied dataset to achieve good recognition rates and incrementally add new people to the database.


Grasping \cite{montesano12actbetas} and affordances \cite{macl08affTRO} is indeed one of the best examples where having a robot acting actively in an environment will provide very meaningful information. Prior works based on learning strategies include tool usage \cite{Stoytchev2005}, grasping \cite{Baier-Lowenstein07rlgrasp}, poking objects \cite{metta03poking} or interactions between objects \cite{Fritz2006}, learning objects categories from affordances \cite{griffith2009toward} and extended to sound categories \cite{sinapov2009interactive}, .


active perception \cite{filliat2000active,holub2008entropy}
\cite{Davison05ICCV,Vidal06ICRA,medusa94jasv,jagersand96onlinejacest}


Other methods add noise on the policy parameters to enforce a larger exploration \cite{stulp2012policy}. In this setting the exploration is more explicit but frequently it is difficult to predict the safety of even small perturbation on the parameters \cite{}. Under joint space exploration it is interesting to note that the typical spino-exterior exploration can be just a side-effect of the optimization and learning process \cite{stulp2012emergent}.
